Low-Rank+Sparse Tensor Compression for Neural Networks

Low-rank tensor compression has been proposed as a promising approach to reduce the memory and compute requirements of neural networks for their deployment on edge devices. Tensor compression reduces the number of parameters required to represent a neural network weight by assuming network weights possess a coarse higher-order structure. This coarse structure assumption has been applied to compress large neural networks such as VGG and ResNet. However modern state-of-the-art neural networks for computer vision tasks (i.e. MobileNet, EfficientNet) already assume a coarse factorized structure through depthwise separable convolutions, making pure tensor decomposition a less attractive approach. We propose to combine low-rank tensor decomposition with sparse pruning in order to take advantage of both coarse and fine structure for compression. We compress weights in SOTA architectures (MobileNetv3, EfficientNet, Vision Transformer) and compare this approach to sparse pruning and tensor decomposition alone.

==> figs/bayesian_model_figures.tex <==
\begin{figure}[t]
%\centering
  \begin{subfigure}[b]{0.25\textwidth}
  \centering
  \input{figs/cp_graphical}    
  \caption{\label{fig: cp graphical}} 
  \end{subfigure}
  \quad\quad
   \begin{subfigure}[b]{0.26\textwidth}
  \centering
    \input{figs/tucker_graphical}    
  \caption{\label{fig: tucker graphical}} 
  \end{subfigure}
\hspace{0.2in}
   \begin{subfigure}[b]{0.38\textwidth}
  \centering
 \raisebox{0.2cm}{\input{figs/tt_graphical}}
  \caption{\label{fig: TT/TTM graphical}} 
  \end{subfigure}
  \caption{(a) CP graphical model (b) Tucker graphical model (c) TT/TTM graphical model. \label{fig: prior description}}
\end{figure}

==> figs/cp_graphical.tex <==
\begin{tikzpicture}

  % Define nodes
  \node[latent]                               (A) {$\ten{A}$};
  \node[latent, above=of A, xshift=0.0cm,yshift=0.4cm] (U) {$\fm{n}$};
  \node[latent, above=of U, xshift=0.0cm,yshift=0.4cm]  (lambda) {$\boldsymbol{\lambda}$};

  % Connect the nodes
  \edge {lambda} {U} ; %
  \edge {U} {A} ; %

  % Plates
  \tikzset{plate caption/.append style={below right=25pt and 20pt of #1.north west}}
  \plate  [inner sep=0.35cm] {uplate} {(U)} {\footnotesize{$1\leq n\leq d$}};

\end{tikzpicture}
%\endpgfgraphicnamed

==> figs/tt_graphical.tex <==
\begin{tikzpicture}
[latent/.append style={minimum size=0.7cm}]
  % Define nodes
  \node[latent]                               (A) {$\ten{A}$};
  \node[latent, above=of A, xshift=0.0cm] (U) {$\ft{n}$};
  \node[latent, above=of U, xshift=0.0cm]  (lambda) {$\rp{n}$};
  \node[latent, above=of A, xshift=1.5cm]  (penultimate_factor) {$\ft{\text{\tiny{$d$-1}}}$};
  \node[latent, above=of A, xshift=2.7cm]  (last_factor) {$\ft{d}$};
  \node[latent, above=of penultimate_factor, xshift=0.6cm] (last_lambda) {$\rp{\text{\tiny{$d$-1}}}$};
  % Connect the nodes
  \edge {lambda} {U} ; %
  \edge {last_lambda} {penultimate_factor,last_factor} ; %
  \edge {U,penultimate_factor,last_factor} {A} ; %
%  \edge {} {A} ; %
  % Plates
  \tikzset{plate caption/.append style={above left=10pt and -20pt of #1.north west}}
  \plate  [inner sep=0.1cm] {uplate} {(U) (lambda)} {\footnotesize{$1\leq n\leq d-2$}};
\end{tikzpicture}
%\endpgfgraphicnamed

==> figs/tucker_graphical.tex <==
\begin{tikzpicture}

  % Define nodes
  \node[latent]                               (A) {$\ten{A}$};
  \node[latent, above=of A, xshift=0.0cm] (U) {$\fm{n}$};
  \node[latent, above=of U, xshift=0.0cm]  (lambda) {$\rp{n}$};
  \node[latent, above=of A, xshift=-1.4cm]  (core) {$\ten{G}$};

  % Connect the nodes
  \edge {lambda} {U} ; %
  \edge {U} {A} ; %
  \edge {core} {A} ; %

  % Plates
  \tikzset{plate caption/.append style={above right=10pt and 0pt of #1.north west}}
  \plate  [inner sep=0.25cm] {uplate} {(U) (lambda)} {\footnotesize{$1\leq n\leq d$}};

\end{tikzpicture}
%\endpgfgraphicnamed
